Quarks: A Secure and Decentralized Blockchain-Based Messaging Network

In last two decades, messaging systems have gained widespread popularity both in the enterprise and consumer sectors. Many of these systems used secure protocols like end-to-end encryption to ensure strong security in one-to-one communication. However, the majority of them rely on centralized servers, which allows them to use their users' personal data. Also, it allows the government to track and regulate their citizens' activities, which poses significant threats to "digital freedom". Also, these systems have failed to achieve security attributes like confidentiality, integrity, and privacy for group communications. In this paper, we present a novel blockchain-based secure messaging system named Quarks that overcomes the security pitfalls of the existing systems and eliminates centralized control. We have analyzed our architecture with security models to demonstrate the system's reliability and usability. We have developed a Proof of Concept (PoC) of the Quarks system leveraging Distributed Ledger Technology (DLT) and conducted load testing on that. We noticed that our PoC system achieves all the desired attributes that are prevalent in a traditional centralized messaging scheme despite the limited capacity of the development and testing environment. Therefore, this assures us of the applicability of such systems in the near future if scaled up properly.

==> tex/discussion.tex <==
% \section{Discussion}
% \label{sec:discussion}
% We have demonstrated our findings of our proposal of decentralising the instant messaging services using blockchain throughout this article. We have made clear our motivation, outline of the the proposal, and demonstrated the architecture along with protocol flows. Furthermore, we have implemented a proof-of-concept and analysed it's performance. In this section, we will explain how our system have satisfied different functional and security requirements (Section \ref{sec:requirement_analysis}). Furthermore, we also discuss its advantages and limitations (Section \ref{subsec:advantages}) along with possible scopes for any future work (Section \ref{subsec:future}). 

% \subsection{Analyzing Requirements}
% As discussed the functional and non-functional requirements of the system in Section \ref{sec:requirement_analysis}, we found that our implemented network was able meet them all. The network maintained the integrity of the sent messages and only the authorized members were able to read and write messages. Furthermore, the nodes synchronized only the messages that they are part of.

% \subsection{Advantages \& Disadvantages}
% \label{subsec:advantages}
% Blockchain is no silver bullet. Our efforts to make a reliable instant messaging system with blockchain has taught us many valuable lessons. Let's shed a light on the pros and cons of Quarks here.

% \subsubsection{Advantages}
% The architecture of Quarks ensures
% \begin{itemize}
%     \item \textsc{Integrity of the messages:} Quarks nodes maintains the message threads in separate distributed ledgers. If any malicious node tries to tamper with ledger, other nodes will detect the tampering effort easily and discard the tampered blocks. Consequently, every message's integrity is ensured. 
%     \item \textsc{Data-ownership for the user:} Quarks network ensures the conversation data is showed only to the authorized users. The blocks of the ledger is kept encrypted and the data only can be retrievable by the member of that message channel. This authorization is ensured through smart-contract.
%     \item \textsc{Trust in the federation:} The trust in the federation between the Quarks nodes has been ensured through the integration of DLT. Smart-contracts of the ledgers are open to every Quarks node. This establishes transparency in the federation. Furthermore, every new messages or block must be validated through smart-contract by majority of the nodes.
%     \item \textsc{No single-point of failure:} As the Quarks network is distributed, it mitigates single point of failure. Each ledger is hosted by the participating nodes of that channel. So, if one node gets unavailable or even destroyed completely, the network will be able to operate without any problem. Furthermore, the affected node will be able to sync with other nodes as soon as it gets available.
%     \item \textsc{Privacy:} Every message is private and the conversation of a message thread is kept in a separate ledger in encrypted manner. This keeps the conversation private from unauthorized entities.
%     \item \textsc{Non-repudiation:} Every message gets validated and endorsed by the Quarks node. These endorsements makes the message non-repudiable.
% \end{itemize}

% \subsubsection{Disadvantages}
% \label{subsubsec:disadvantages}
% As CAP theorem\cite{brewer2000CAP} suggests, we had to chose between availability and consistency during a partition of network happens. As we analyzed our architecture and implementation, we saw that Quarks is much slower than traditional centralized system. During designing our network we prioritized the consistency and reliability of every single messages.

% The disadvantages,
% \begin{itemize}
%     \item \textsc{Low Throughput:} Quarks was built by leveraging distributed ledger technology. Every block or messages must be verified through smart contracts by participating nodes of that channel. For this reason, a send message from a user causes multiple network calls between Quarks nodes to ensure the new messages authenticity, validity, and security. These network calls between nodes helps nodes to reach consensus on that new message. Consequently, a message need some time to reach finality. This results in lower throughput for the system.
%     \item \textsc{Nodes availability is indispensable:} Quarks nodes maintain a separate ledger and smart-contract for each conversation or message thread. As each sent message must be verified by the majority of the nodes of that channel, the availability of the Quarks node is essential for successful instant messaging.
% \end{itemize}

% \subsection{Future Work}
% \label{subsec:future}
% As per our knowledge, this work is the first effort to make an instant messaging network using distributed ledger technology. From our evaluation (Section \ref{sec:evaluation}) we found that Quarks is not high-performing as traditional centralized architecture. However, this was expected from Quarks, as discussed in Section \ref{subsubsec:disadvantages}. These disadvantages points direction to our next goal for Quarks.

% \begin{itemize}
%     \item \textsc{Enhance performance of PoC:} As discussed in section \ref{sec:implementation}, we implemented our PoC using Hyperledger Fabric. We want to explore other permissioned blockchain frameworks like R3 Corda \cite{brown2018corda}, EOSIO \cite{eosio}, and Quorum \cite{quorum}. However, the architecture of the Permissioned blockchain frameworks are designed and implemented such way so that everyone can use it for various purposes. Which may create bottlenecks for our implementation. As our protocols for Quarks has been defined in (Section \ref{subsec:protocol}, we want to implement our PoC from scratch. This will give us the upperhand to optimize according to the need of the protocol.
%     \item \textsc{Develop Test Network:} Upon getting satisfying results from the PoCs, we plan to move to the system design and development of the Quarks testnet. Quarks Network is open-source and will be kept that way. 
%     \item \textsc{Deploy Main Network:} If our test network gets a success, we will deploy Quarks Main network. Everyone will be able participate in the network and get benefit from it. 
% \end{itemize}

% If you want to contribute to Quarks. Please feel free to explore our repository at \textit{https://github.com/probaaho/quarks-network}



==> tex/security_analysis.tex <==
\subsection{Informal Security analysis of \texttt{Quarks}}
\label{security_analysis}
\textbf{Confidentiality.} Every message in the ledger in \texttt{Quarks} is encrypted with a secret key unique to a channel. This channel's secret key is only known to the members of the channel. This guarantees protection against potential data breaches. \\
\textbf{Integrity.} In \texttt{Quarks} all the messages are stored on-chain. That means it is impossible to delete or tamper the previous messages. \\
\textbf{Non-Repudiation.} As every message-write is digitally signed by the members and signatures are being verified by smart contract, Quarks diminishes repudiation attempts. \\
\textbf{Authentication and Authorization.} Users interact with the \texttt{Quarks} by authenticating with their private keys which enables the \texttt{Quarks} nodes to prevent unauthorized access to the users’ data. \\
\textbf{Resilient to DDoS Attacks.} DDoS attackers may successfully make a single node unavailable for some time; however, the decentralized nature of the \texttt{Quarks} network will keep the service intact. 

